What's Behind the Couch? Directed Ray Distance Functions (DRDF) for 3D Scene Reconstruction

We present an approach for full 3D scene reconstruction from a single unseen image. We train on dataset of realistic non-watertight scans of scenes. Our approach predicts a distance function, since these have shown promise in handling complex topologies and large spaces. We identify and analyze two key challenges for predicting such image conditioned distance functions that have prevented their success on real 3D scene data. First, we show that predicting a conventional scene distance from an image requires reasoning over a large receptive field. Second, we analytically show that the optimal output of the network trained to predict these distance functions does not obey all the distance function properties. We propose an alternate distance function, the Directed Ray Distance Function (DRDF), that tackles both challenges. We show that a deep network trained to predict DRDFs outperforms all other methods quantitatively and qualitatively on 3D reconstruction from single image on Matterport3D, 3DFront, and ScanNet.

==> sections/supp_baselines.tex <==
One of the key challenges of


\parnobf{Unsigned Distance Function}


\parnobf{Sign-Agnostic Loss}

\parnobf{Occupancy Function}


==> sections/supp_decoding.tex <==
\dfnote{Not sure this goes here. This can almost certainly fit in the main paper when explaining the baselines }

We report the design decisions used in the baselines and our method. Throughout, let $S$ denote a set of surface intersections along a ray.

\parnobf{Unsigned Distance Function (UDF)}

The UDF $\min_{s \in S} |z-s|$ still has a minimum and derivative sign-change at the intersection under expectation. We aim to use ths.

\parnoit{Direct Thresholding} We look for the zero-crossings of $\hat{d}_U(z;s) - \tau$ for varying $\tau$.

\parnoit{Gradient Zero-Crossing} Since the expected UDF still changes its derivative's sign at the intersection, we compute numerical derivatives and locate zero-crossings.

\parnoit{Thresholding with Non-Maximum Suppression} \dfnote{what}

\parnobf{Sign Agnostic Learning (SAL)} Since SAL produces a signed distance function, we look for zero-crossings.

\parnobf{Occupancy Function (OF)}
The OF $d_O = (\min_{s \in S} |z-s|) < r$ has a binarization parameter, namely the radius $r$. We optimize $r$ on the validation set (for $1$m, $0.5$m, $0.25$m, $0.1$m). 

\parnoit{Thresholding} Following \cite{saito2019pifu}, we find zero-crossings of $\hat{d}_O(z;s)-0.5$ for the predicted distance $\hat{d}_O$. However, since these include both entrances and exits to the $r$-ball at the intersection, we only include positive-to-negative zero-crossings to avoid repeated phantom intersections.

\parnoit{Peak-Finding} Since the expected function still has a peak at the intersection, we find peaks using \dfnote{what}.

\parnoit{Averaging Entrances and Exits} The first thresholding approach induces a bias in the predictions: the intersections are all systematic underestimates. We correct this by pairing adjacent positive-to-negative and negative-to-positive zero-crossings that could represent the adjacent zero-crossings of an intersection (correct order, distance), and average them.

\parnobf{Directed Ray Distance Function (DRDF)}
For the DRDF, we simply look for zero-crossings.


==> sections/supp_proof.tex <==



==> supp_sections/interactive_demo.tex <==


\subsection{Approach Overview}
We show an overview of the approach in \texttt{approach\_overview.webm}. It discusses the challenges in designing a single image to 3D system trained on real 3D scene data and presents our approach briefly.
% $\bullet$ . We describe the overview of our approach in a {\it 5 minute} video. We discuss the challenges and our approach from the paper.\\
\subsection{Video Results}
\label{sec:video}
We provide {\it three} video files with results from our models. These videos show the outputs of our model
and compare them to the ground truth and baselines by showing salient features at different instances in video frames. All the videos files are best viewed a web-browser\\
\noindent
$\bullet$ \texttt{result\_videos/main\_paper.mp4}. Shows the qualitative results from Fig 6, and Fig 7 of the main paper in order of their appearance. We highlight salient regions our model similar to the zoom-ins in the main paper to qualitatively compare the outputs. The first part of the video compares the DRDF outputs with ground truth and the second part of the video compares against various baselines. This video contains {\it all} the qualitative examples in the main paper.\\
$\bullet$ \texttt{result\_videos/additional.mp4}. This video shows additional qualitative examples in addition to the main qualitative examples shown. It is also divided into two parts where the first part compares against ground truth while the second part compares against outputs of other baseline methods.\\
$\bullet$ \texttt{result\_videos/supp\_qual.mp4}. This video shows six samples from the qualitative figures shown in the supplemental in \figref{fig:matterport_novel}, \ref{fig:threedf_novel}, \ref{fig:scannet_novel} (2 samples from each dataset) and compares the outputs against the ground truth.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{suppfigures/video.jpg}
    \caption{{\bf Qualitative Video.} Screen Capture from \texttt{main\_paper.mp4}. Our video shows model outputs and a highlight box (red/black) describing regions of interest and salient differences between methods. Our supplementary contains three videos of results each showcasing a different set of examples. a) \texttt{main\_paper.mp4} has all the results from the main paper and we highly encourage watching this. b) \texttt{additional.mp4} has more result showcasing performance with respect to other baselines, and ground-truth c) \texttt{supp\_qual.mp4} has video results for samples in the supplementary PDF}. 
 \end{figure}



\subsection{Interactive Demo}
\label{sec:interactive_demo}
We provide three outputs of DRDF from the main paper and  embed them inside the HTML as an interactive demo to qualitatively assess our outputs and compare against the GT. The demo allows us to view the outputs from the given input image (left most column on the demo) and compare with GT(middle column on the demo) with the prediction (right most column on the demo)
Inside the folder \texttt{interactive\_demo} is a file \texttt{model\_vis.html}. Open this file in a web browser (best viewed in Google Chrome or Firefox) to see the interactive demo of the output from our model.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{suppfigures/demo.jpg}
    \caption{{\bf Interactive Demo.} Screen Capture of interactive demo. We present an interactive demo of selected outputs from the main paper, allowing explorations from more camera view-points not explored completely in the video trajectory. Please open the \texttt{model\_vis.html} in your web-browser (works best with Google Chrome and Firefox).}
\end{figure}





